Transducer Tuning: Efficient Model Adaptation for Software Tasks Using Code Property Graphs

Large language models have demonstrated promising performance across various software engineering tasks. While fine-tuning is a common practice to adapt these models for downstream tasks, it becomes challenging in resource-constrained environments due to increased memory requirements from growing trainable parameters in increasingly large language models. We introduce \approach, a technique to adapt large models for downstream code tasks using Code Property Graphs (CPGs). Our approach introduces a modular component called \transducer that enriches code embeddings with structural and dependency information from CPGs. The Transducer comprises two key components: Graph Vectorization Engine (GVE) and Attention-Based Fusion Layer (ABFL). GVE extracts CPGs from input source code and transforms them into graph feature vectors. ABFL then fuses those graphs feature vectors with initial code embeddings from a large language model. By optimizing these transducers for different downstream tasks, our approach enhances the models without the need to fine-tune them for specific tasks. We have evaluated \approach on three downstream tasks: code summarization, assert generation, and code translation. Our results demonstrate competitive performance compared to full parameter fine-tuning while reducing up to 99\% trainable parameters to save memory. \approach also remains competitive against other fine-tuning approaches (e.g., LoRA, Prompt-Tuning, Prefix-Tuning) while using only 1.5\%-80\% of their trainable parameters. Our findings show that integrating structural and dependency information through Transducer Tuning enables more efficient model adaptation, making it easier for users to adapt large models in resource-constrained settings.

==> backup/name.tex <==
Prior studies have proposed various efficient adaptation techniques, such as Adapter-based \cite{DBLP:conf/emnlp/BapnaF19, DBLP:conf/icml/HoulsbyGJMLGAG19, DBLP:conf/emnlp/PfeifferVGR20, DBLP:conf/emnlp/PfeifferRPKVRCG20, DBLP:conf/eacl/PfeifferKRCG21, DBLP:conf/nips/LiuTMMHBR22, LoRA, DBLP:conf/iclr/Hyeon-WooYO22, DBLP:conf/iclr/YehHGYO024, DBLP:journals/corr/abs-2202-13914, DBLP:conf/iclr/KopiczkoBA24} and Prompt-based \cite{PrefixTuning, PromptTuning, DBLP:conf/acl/LiuJFTDY022} approaches to address the memory requirement challenge. Adapter-based methods \cite{DBLP:conf/emnlp/BapnaF19, DBLP:conf/icml/HoulsbyGJMLGAG19, DBLP:conf/emnlp/PfeifferVGR20, DBLP:conf/emnlp/PfeifferRPKVRCG20, DBLP:conf/eacl/PfeifferKRCG21, DBLP:conf/nips/LiuTMMHBR22, LoRA, DBLP:conf/iclr/Hyeon-WooYO22, DBLP:conf/iclr/YehHGYO024, DBLP:journals/corr/abs-2202-13914, DBLP:conf/iclr/KopiczkoBA24} introduce additional trainable parameters into a language model and update only these parameters during the fine-tuning stage rather than the entire model. On the other hand, embedding-based methods \cite{PrefixTuning, PromptTuning, DBLP:conf/acl/LiuJFTDY022} modify the output of the embedding layer before feeding it to the initial encoder/decoder layer of the model. 

Despite their effectiveness in reducing memory requirements, none of these efficient fine-tuning approaches leverage the rich structural and dependency information inherent in source code. Code is different from natural language text, where it has well-defined structures, dependencies, and control flows that can be explicitly represented using graphs. Therefore, treating source code merely as a sequence of tokens during fine-tuning may limit the model's ability to capture important patterns and relationships in code.

In this work, we propose a novel approach that enhances efficient fine-tuning techniques by incorporating structural information from source code through graph-based representations. Unlike sequential representations, graphs can naturally capture long-range dependencies and relationships between program elements - for instance, connecting variable declarations with their uses, or representing control flow relationships that may span across many lines in the sequential representation. By leveraging these structural insights during the fine-tuning process, we aim to help models better understand and reason about code while maintaining the memory efficiency benefits of existing adaptation techniques.


In this work, we propose enhancing these fine-tuning approaches by incorporating the structural information of source code through graph-based representation during the fine-tuning stage.


Graph-based representations offer several advantages over purely sequential approaches. For instance, while two dependent variables may appear far apart in a linear sequence, a graph can represent their relationship more directly, making these dependencies more apparent to the model. Furthermore, graphs can effectively encode control flow and other structural patterns that are fundamental to program understanding. This insight motivates our proposal to use structural information from graph to efficiently fine-tune language models.




—typically represented using graphs—we can potentially achieve comparable performance with even fewer trainable parameters during the fine-tuning stage. This graph-based approach could offer a promising direction for further reducing the parameter footprint while maintaining the strong performance of current adaptation techniques.

One drawback of the aforementioned approaches is they do not take advantage of the inherent structure, control flow, and dependencies information within source code. This information, typically represented using graphs, offers a more accurate depiction of source code than just simple sequences. By leveraging this information, we believe that language models can potentially achieve a better understanding of source code using fewer trainable parameters during the fine-tuning stage while minimizing performance degradation due to the reduced trainable parameters.

==> backup/old_table.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{llccccccccc}
\hline
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Tuning Method}} & \textbf{Summarization} & \textbf{Assert Generation} & \textbf{Code Translation} & \textbf{Code Repair} \\
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}p{1cm}@{}}CodeT5+\\\centering 220M\end{tabular}} 
    & Transducer Tuning & 99.84 $\pm$ 0.21 & 82.32 $\pm$ 0.30 & 96.60 $\pm$ 1.31 & 98.10 $\pm$ 0.39 \\
    & No Finetuning      & 95.49 $\pm$ 0.00 & 76.85 $\pm$ 0.00 & 94.47 $\pm$ 0.00 & 96.00 $\pm$ 0.00 \\
    & Full Finetuning    & 99.91 $\pm$ 0.01 & 83.16 $\pm$ 0.01 & 97.78 $\pm$ 0.00 & 99.87 $\pm$ 0.00 \\
    & Linear Adapter     & 98.05 $\pm$ 0.88 & 82.48 $\pm$ 0.02 & 97.70 $\pm$ 0.12 & 99.31 $\pm$ 0.71 \\
    & LoRA               & 99.91 $\pm$ 0.00 & 83.17 $\pm$ 0.00 & 97.78 $\pm$ 0.00 & 99.87 $\pm$ 0.00 \\
    & Prefix-Tuning      & 99.93 $\pm$ 0.01 & 83.17 $\pm$ 0.00 & 97.78 $\pm$ 0.00 & 99.87 $\pm$ 0.00 \\
    & Prompt-Tuning      & 99.91 $\pm$ 0.01 & 83.17 $\pm$ 0.00 & 94.40 $\pm$ 0.27 & 97.46 $\pm$ 1.13 \\
\hline
\multirow{7}{*}{\begin{tabular}[c]{@{}p{1cm}@{}}CodeT5+\\\centering 770M\end{tabular}} 
    & Transducer Tuning & 98.11 $\pm$ 1.61 & 81.16 $\pm$ 0.71 & 94.88 $\pm$ 0.08 & 96.75 $\pm$ 3.94 \\
    & No Finetuning      & 87.90 $\pm$ 0.00 & 74.13 $\pm$ 0.00 & 90.10 $\pm$ 0.00 & 95.71 $\pm$ 0.00 \\
    & Full Finetuning    & 99.81 $\pm$ 0.01 & 83.16 $\pm$ 0.01 & 97.78 $\pm$ 0.00 & 99.87 $\pm$ 0.00 \\
    & Linear Adapter     & 98.24 $\pm$ 1.39 & 81.23 $\pm$ 0.88 & 97.77 $\pm$ 0.02 & 99.82 $\pm$ 0.02 \\
    & LoRA               & 99.79 $\pm$ 0.02 & 83.17 $\pm$ 0.00 & 97.78 $\pm$ 0.00 & 99.87 $\pm$ 0.00 \\
    & Prefix-Tuning      & 99.85 $\pm$ 0.00 & 83.15 $\pm$ 0.02 & 97.78 $\pm$ 0.00 & 99.87 $\pm$ 0.00 \\
    & Prompt-Tuning      & 99.82 $\pm$ 0.01 & 83.17 $\pm$ 0.00 & 90.15 $\pm$ 0.01 & 99.22 $\pm$ 0.71 \\
\hline
\end{tabular}
\caption{Performance comparison across different tuning methods for various tasks. \approach yields significant improvement against No Fine-tuning and competitive performance against other tuning baselines. The standard deviations represent the variability across two trials, each conducted with a different random seed.}
\label{tab:performance-result}
\end{table}

\begin{table}[ht]
\centering

\begin{tabular}{ccccccc}
\hline
\textbf{Model} & \textbf{Transducer} & \textbf{Full Finetuning} & \textbf{LoRA} & \textbf{Linear Adapter} & \textbf{Prefix-Tuning} & \textbf{Prompt-Tuning} \\
\hline
CodeT5+ 220M & 3.52 & 4.48 & 4.48 & 3.68 & 4.49 & 3.03 \\
CodeT5+ 770M & 5.76 & 8.20 & 8.19 & 8.20 & 8.20 & 6.13 \\
\hline
\end{tabular}
\caption{Average improvement against No Fine-tuning across different tuning methods. Higher is better.}
\label{tab:vs-noft}
\end{table}

\begin{table*}[ht]
\centering

\begin{tabular}{clrrrrr}
\hline
\multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Tuning Method}} & \textbf{Summarization} & \textbf{Assert Generation} & \textbf{Code Translation} & \textbf{Code Repair} & \textbf{Average} \\
\hline
\multirow{6}{*}{\begin{tabular}[c]{@{}p{1cm}@{}}CodeT5+\\\centering 220M\end{tabular}} & Transducer Tuning & 30,728 & 30,728 & 30,728 & 30,728 & 30,728 \\
                              & Full Fine-tuning    & 222,882,048 & 222,882,048 & 222,882,048 & 222,882,048 & 222,882,048 \\
                              & Linear Adapter      & 589,824 & 589,824 & 589,824 & 589,824 & 589,824 \\
                              & LoRA                & 884,736 & 442,368 & 884,736 & 442,368 & 663,552 \\
                              & Prefix-Tuning       & 184,320 & 921,600 & 184,320 & 921,600 & 552,960 \\
                              & Prompt-Tuning       & 38,400 & 76,800 & 38,400 & 76,800 & 57,600 \\
\hline
\multirow{6}{*}{\begin{tabular}[c]{@{}p{1cm}@{}}CodeT5+\\\centering 770M\end{tabular}} & Transducer Tuning & 37,128 & 37,128 & 37,128 & 37,128 & 37,128 \\
                              & Full Fine-tuning    & 737,639,424 & 737,639,424 & 737,639,424 & 737,639,424 & 737,639,424 \\
                              & Linear Adapter      & 1,048,576 & 1,048,576 & 1,048,576 & 1,048,576 & 1,048,576 \\
                              & LoRA                & 2,359,296 & 1,179,648 & 2,359,296 & 1,179,648 & 1,769,472 \\
                              & Prefix-Tuning       & 491,520 & 491,520 & 491,520 & 1,228,800 & 675,840 \\
                              & Prompt-Tuning       & 102,400 & 102,400 & 102,400 & 102,400 & 102,400 \\
\hline
\end{tabular}
\caption{Trainable parameter count comparison across different tuning methods. \approach leverages the fewest trainable parameters among all tuning methods. LoRA, Prefix-Tuning, and Prompt-Tuning can have different parameter counts for different tasks due to different tuned hyperparameters.}
\label{tab:parameter-result}
\end{table*}


\begin{table*}[ht]
\centering

\begin{tabular}{llcccccccc}
\hline
\textbf{Model} & \multicolumn{1}{c}{\textbf{Variant}} & \textbf{Summarization} & \textbf{Assert Generation} & \textbf{Code Translation} & \textbf{Code Repair} \\
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}p{1cm}@{}}CodeT5+\\\centering 220M\end{tabular}}  
    & GVE + ABF      & \textbf{99.84} $\pm$ 0.21 & 82.32 $\pm$ 0.30 & \textbf{96.60} $\pm$ 1.31 & 98.10 $\pm$ 0.39 \\
    & GVE-only   & 99.31 $\pm$ 0.06 & \textbf{83.14} $\pm$ 0.04 & 96.03 $\pm$ 0.00 & 99.37 $\pm$ 0.09 \\
    & ABF-only   & 94.33 $\pm$ 7.32 & 77.07 $\pm$ 8.62 & 92.53 $\pm$ 2.65 & 97.48 $\pm$ 3.38 \\
    & Linear   & 99.54 $\pm$ 0.09 & 83.08 $\pm$ 0.07 & 91.76 $\pm$ 0.36 & \textbf{99.45} $\pm$ 0.59 \\
\hline
\multirow{4}{*}{\begin{tabular}[c]{@{}p{1cm}@{}}CodeT5+\\\centering 770M\end{tabular}} 
    & GVE + ABF      & 98.11 $\pm$ 1.61 & 81.16 $\pm$ 0.71 & 94.88 $\pm$ 0.08 & 96.75 $\pm$ 3.94 \\
    & GVE-only   & 96.23 $\pm$ 1.55 & 78.79 $\pm$ 2.51 & \textbf{97.78} $\pm$ 0.00 & \textbf{99.54} $\pm$ 0.12 \\
    & ABF-only   & 98.64 $\pm$ 0.52 & \textbf{83.16} $\pm$ 0.01 & 91.11 $\pm$ 0.33 & 94.33 $\pm$ 4.16 \\
    & Linear   & \textbf{99.17} $\pm$ 0.42 & 79.31 $\pm$ 4.64 & 90.40 $\pm$ 0.02 & 93.27 $\pm$ 0.88 \\
\hline
\end{tabular}
\caption{Ablation study results showing the impact of different components in \approach on model performance across various tasks. The table compares the default setting (GVE + ABF) with three other variants: GVE-only, ABF-only, and Linear. Results indicate the significance of using information from CPGs and processing it using GNN layer to enhance model performance.}
\label{tab:ablation}
\end{table*}
